Body Design and Gait Generation of Chair-Type Asymmetrical Tripedal Low-rigidity Robot

In this study, a chair-type asymmetric tripedal low-rigidity robot was designed based on the three-legged chair character in the movie "Suzume" and its gait was generated. Its body structure consists of three legs that are asymmetric to the body, so it cannot be easily balanced. In addition, the actuator is a servo motor that can only feed-forward rotational angle commands and the sensor can only sense the robot's posture quaternion. In such an asymmetric and imperfect body structure, we analyzed how gait is generated in walking and stand-up motions by generating gaits with two different methods: a method using linear completion to connect the postures necessary for the gait discovered through trial and error using the actual robot, and a method using the gait generated by reinforcement learning in the simulator and reflecting it to the actual robot. Both methods were able to generate gait that realized walking and stand-up motions, and interesting gait patterns were observed, which differed depending on the method, and were confirmed on the actual robot. Our code and demonstration videos are available here: https://github.com/shin0805/Chair-TypeAsymmetricalTripedalRobot.git

==> preamble.tex <==
\RequirePackage[l2tabu, orthodox]{nag} % 古いコマンドやパッケージの利用を警告する
\usepackage[all, warning]{onlyamsmath} % amsmath が提供しない数式環境を使用した場合に警告
% for not arxiv
% \usepackage[dvipdfmx]{color}
% \usepackage[dvipdfmx,bookmarks=true,bookmarksnumbered=true,bookmarkstype=toc,%
%      colorlinks=true,%
%      linkcolor=black, %%追加20090108
%      citecolor=black, %%追加20090108
%      urlcolor=black, %%追加20090108
%      bookmarksopen=true,%しおりツリーをデフォルトで開く
% %     backref=page,%citeにどこで使っているか出るようになる
%      pdftitle=\PDFTITLE,%
%      pdfsubject=\PDFSUBJECT,%
%      pdfauthor=\PDFAUTHOR,%
%      pdfkeywords=\PDFKEYWORDS]{hyperref}
% %% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvips]{graphicx}
% \usepackage[dvipdfmx]{}

% for arxiv
\usepackage{hyperref}
\usepackage{color}
\usepackage{graphicx}

% \usepackage{jtygm}
\usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
\usepackage{txfonts,mathptmx}

%%%% カスタマイズしたい場合は以下に書く

\newcommand{\TODO}[1]{\fbox{{\textbf TODO:}#1}}
\usepackage{layout}
\usepackage{wrapfig}

% \usepackage{pxjahyper}
% hypcap: figref, tabrefしたときにジャンプ先がキャプション部ではなく図の上になる
\usepackage[figure,figure*,table,table*]{hypcap}
% \usepackage{eclbkbox}
%% \usepackage[dvipdfmx]{graphicx}
% \usepackage[dvipdfmx]{}
\usepackage{url} % \url のために必要
%% \url{http://nile.ulis.ac.jp/~yuka/}
%\usepackage{html} % latex2html で 利用
\usepackage{algorithm}
\usepackage{algcompatible}
\usepackage{algpseudocode}
\usepackage{amsmath}
\algblockdefx{FORP}{ENDFORP}[1]%
  {\textbf{for}#1 \textbf{do in parallel}}%
  {\textbf{end for}}
\algnewcommand{\algorithmicand}{\textbf{ and }}
\algnewcommand{\algorithmicor}{\textbf{ or }}
\algnewcommand{\OR}{\algorithmicor}
\algnewcommand{\AND}{\algorithmicand}
% \usepackage[subrefformat=parens]{subcaption}
% \captionsetup{compatibility=false} % http://www.yamamo10.jp/yamamoto/comp/latex/make_doc/insert_fig/
% \captionsetup[sub]{skip=4pt}

%% \newcommand{\tabref}[1]{{表~\ref{#1}}~}
%% \newcommand{\figref}[1]{{図~\ref{#1}}~}
%% \newcommand{\equref}[1]{{式(\ref{#1})}~}
\newcommand{\secref}[1]{Section \ref{#1}}
\newcommand{\subsecref}[1]{Subsection \ref{#1}}
\newcommand{\tabref}[1]{{Table \ref{#1}}}
\newcommand{\figref}[1]{{Fig. \ref{#1}}}
%% \newcommand{\figref}[1]{\figurename\ref{fig:#1}}
\newcommand{\equref}[1]{{Eq. \ref{#1}}}
\newcommand{\algoref}[1]{{Alg. \ref{#1}}}
\newcommand{\enumref}[1]{{\ref{#1}}}
%% \renewcommand{\figurename}{Fig.}
%% \renewcommand{\tablename}{Table }

\newcommand{\switchlanguage}[2]{%
  \ifx\paperlanguage\empty%
  #1%
  \else%
  #2%
  \fi%
}

